Single-Shot Clothing Category Recognition in Free-Configurations with Application to Autonomous Clothes Sorting

This paper proposes a single-shot approach for recognising clothing categories from 2.5D features. We propose two visual features, BSP (B-Spline Patch) and TSD (Topology Spatial Distances) for this task. The local BSP features are encoded by LLC (Locality-constrained Linear Coding) and fused with three different global features. Our visual feature is robust to deformable shapes and our approach is able to recognise the category of unknown clothing in unconstrained and random configurations. We integrated the category recognition pipeline with a stereo vision system, clothing instance detection, and dual-arm manipulators to achieve an autonomous sorting system. To verify the performance of our proposed method, we build a high-resolution RGBD clothing dataset of 50 clothing items of 5 categories sampled in random configurations (a total of 2,100 clothing samples). Experimental results show that our approach is able to reach 83.2\% accuracy while classifying clothing items which were previously unseen during training. This advances beyond the previous state-of-the-art by 36.2\%. Finally, we evaluate the proposed approach in an autonomous robot sorting system, in which the robot recognises a clothing item from an unconstrained pile, grasps it, and sorts it into a box according to its category. Our proposed sorting system achieves reasonable sorting success rates with single-shot perception.

==> texfiles/pipeline_copy.tex <==
\subsection{Outline\label{sec:outline}}

\begin{figure*}[th]
\centering
\includegraphics[width= 0.95\textwidth]{./flowchart/pipeline.png}
\caption{The proposed pipeline of clothing category recognition.}
\label{fig:pipeline}
\end{figure*}

We propose a pipeline incorporating a rich visual description of clothing material type attributes. 2.5D Surface textures of clothing are useful for recognising materials types (Fig.\ref{fig:textures}). Among texture recognition approaches, Local Binary Pattern features (LBP) have achieved great success in grey scale texture recognition \cite{lbpPAMI2002}. In this paper, LBP is applied to the high frequency phase of 2.5D clothes surfaces to describe the 2.5D fabric structure. Wrinkles provide another important feature of clothing material, specially in free-configuration settings. Wrinkles can reveal thickness and stiffness attributes of the fabric material. For instance, wrinkles in T-shirts are usually smaller than those of sweaters because of their thickness attributes, whilst jeans usually have fewer wrinkles than other clothing types since denim is stiffer. 

Our recognition pipeline (Fig. \ref{fig:pipeline}) consists of four modules: (1) global and (2) local feature extraction, (3) encoding, and (4) classification. For global features, Shape Index (SI) and LBP descriptors are extracted (Section{~\ref{sec:si}} and Section{~\ref{sec:lbp}}, respectively). We also propose a Topology Spatial Distance (TSD) feature computed from surface topologies (Section{~\ref{sec:tsd}}), which captures the intrinsic properties of wrinkles. For local features, $B$-Spline Patches (BSP) (Section{~\ref{sec:bsp}) are extracted densely on surface ridges and then encoded using sparse coding in order to represent the 2.5D shape of wrinkles. Finally, global and local descriptions are fused together and fed into a classifier in order to learn clothing category models (Section{~\ref{sec:svm}}). 

\subsection{A Generic Clothing Surface Analysis Framework}

In our previous work~\cite{lisun2015icra}, we reported a generic clothing surface analysis framework for garment grasping and flattening in robotic tasks. We further extend this framework in Section~\ref{sec:si}, Section~\ref{sec:tsd} and Section~\ref{sec:bsp}. For completeness, a brief description is given below.

A piece-wise $B$-Spline surface approximation is adapted to fit a continuous implicit surface onto the original depth map (Fig. \ref{fig:pipeline}-d). Surface shape and topology features are derived from low-level surface geometries such as curvature. We estimate maximum curvature and minimum on fitted clothing surface. To detect wrinkles on the garment surface, we compute the surface's topology which includes surface ridges and wrinkle contours (shown as red and green lines in Fig.~\ref{fig:pipeline}-c). We detect ridges by thresholding the maximal curvature at different scales, and the preliminary result is filtered by `ridge' regions (Section~\ref{sec:si}). Wrinkle contours are estimated by computing the zero-crossings of the second derivatives of the garment's surface (further details can be found in \cite{lisun2015icra}). Morphological image operations~\cite{lam1992thinning} are applied to thin ridges and wrinkle contours to obtain ridge topologies of one-pixel-width.

\subsection{Global Features\label{sec:global}}
\subsubsection{Histogram of Shape Index (SI)\label{sec:si}}
Shape Index~\cite{koenderink1992surface} classifies surface regions into real-valued index values $S$ in the range $[-1,1]$. The SI value is quantised into 9 intervals corresponding to 9 surface types -- cup, trough, rut, saddle rut, saddle, saddle ridge, ridge, dome and cap. Amongst shape types, `ridge' (shown as yellow in Fig.~\ref{fig:pipeline}-b) is critical in the analysis and description of wrinkles. The shape index value $S^{p}$ of point $p$ can be calculated as follows~\cite{koenderink1992surface}:
\begin{equation}
\centering
\displaystyle S^{p}= \frac{2}{\pi} \tan^{-1} \left [ \frac {k_{min}^{p}+k_{max}^{p}}{k_{min}^{p}-k_{max}^{p}} \right ],
\label{eq:12}
\end{equation}
where $k_{min}^{p}$ and $k_{max}^{p}$ are the minimal and maximal curvatures at point $p$, respectively. In order to parse shape information exhibited by the visible cloth surface, we calculate the shape index from the $B$-Spline fitted depth map and apply majority rank filtering (Fig. \ref{fig:pipeline}-b). This non-linear filtering removes outlier surface classifications and can be tuned to produce a relatively clean classification of shape types over the cloth surface. Finally, a 9 dimensional histogram of shape indices is constructed and then $L^{2}$ normalisation is applied.

\subsubsection{Histogram of Local Binary Patterns (LBP)\label{sec:lbp}}
We extract local binary patterns over multiple-scales in the raw depth map of the visible clothing surface. All descriptors are quantified into a global histogram. That is, LBP histograms are calculated separately at different scales. In our implementation, a selected collection of patterns (58 patterns) are used~\cite{vedaldi08vlfeat}. For multiple-scale feature extraction, a 3 layered Gaussian pyramid is constructed using a sub-division factor of 2 and a Gaussian smoothing parameter ($\sigma$ = 0.375). A global LBP descriptor of 174 dimensions (58$\times$3) is obtained.

%\begin{figure}[thpb]
%\centering
%\includegraphics[width= 0.45\textwidth]{./images/lbp_patterns.png}
%\caption{In theory, there are 256 ($2^{8}$) LBP patterns for eight positions, in this paper, VlFeat's implementation, 58 more representative patterns are selected for more reliable statistic. In this figure, black block means the depth of its position is smaller than the depth of the center, while white refers the the depth is larger than the center. The strategy of generating these partterns are rotating the white block anti-clockwise direction to get 8 different partterns, then increase the number of white blocks (from 1 to 7) and also rotate anti-clock-wisely to get 7$\times$8 patterns in total. Pulsing two additional patterns, 58 LBP patterns are obtained finally.          }
%\label{fig:lbp_patterns}
%\end{figure}

\subsubsection{Histogram of Topology Spatial Distances (TSD)\label{sec:tsd}}
Having obtained surface topologies (Section~\ref{sec:si}), we estimate wrinkles' magnitude by calculating the distance between each ridge point and its nearest contour points. Given all surface ridge points $R=\{r_{1},...,r_{n_{r}}\}$ and each wrinkle's contour points $W=\{w_{1},...,w_{n_{w}}\}$, the TSD along the $x-y$ plane, $TSD_{i}^{xy}$, and depth direction, $TSD_{i}^{d}$, are calculated as follows: 
\begin{equation}
\centering
TSD_{i}^{xy} = \min_{i\in n_w} \Vert r_{i},w_{j} \Vert^{2}
\end{equation}
\begin{equation}
\centering
TSD_{i}^{d} = d^{r}_{i} - d^{c}_{\arg_{j} \min \Vert r_{i},w_{j} \Vert^{2}},
\end{equation}
where $d^{r}_{i}$ and $d^{w}_{j}$ are the depth value of the $r_{i}$ and $w_{j}$. The TSD description is a bi-dimensional histogram of topological spatial distances $\{TSD_{1}^{xy},...,TSD_{n_{r}}^{xy}\}$ and $\{TSD_{1}^{d},...,TSD_{n_{r}}^{d}\}$, which represents the wrinkles' estimated width and height, respectively. The final TSD description is obtained by vectorising the bi-dimensional histogram. Width values smaller than 5 or larger than 50 are removed. For both $TSD^{xy}$ and $TSD^{d}$ dimensions, bins are set as 10 uniform intervals ranging from 5 to 50. The latter corresponds to the possible range of wrinkle widths and heights -- for $TSD^{xy}$, the unit is pixels, while for $TSD^{d}$ the unit is millimetres. After applying $L^{2}$ normalisation, the final 100 dimensional TSD global descriptor (10$\times$10) is obtained.

\subsection{Local Features}
\subsubsection{Local $B$-Spline Patch (BSP)\label{sec:bsp}}
$B$-Spline surface is a classic 3D surface representation in computer graphics, where the surface shape can be manipulated by a set of control points. In our approach, we adapt $B$-Spline surface fitting to describe local clothing patches. That is, for each $m\times n$ patch $P$ of the depth map, a set of 3D points are given ${X\{x_{1},...,x_{n}\}}$,${Y\{y_{1},...,y_{m}\}}$, $P=\{P_{(x_{1},y_{1})},...,P_{(x_{i},y_{j})},...,P_{(x_{n},y_{m})}\}$, where $x_{i}$,$y_{i}$ are x, y coordinates and $P_{(x_{i},y_{i})}$ is the value of the depth map. The implicit surface can be represented as:
\begin{equation}
P(u,w) = \sum_{i=1}^{n+1}\sum_{j=1}^{m+1} \Omega_{i,j}\alpha_{i,k}(x)\beta_{j,l}(y),
\label{eq:1}
\end{equation}
where $\Omega_{i,j}$ represents the control point at row $i$ and column $j$. $\alpha_{i,k}(x)$ and $\beta_{j,l}(y)$ are the basis functions in the $x-y$ plane, more details of which can be found in~\cite{rogers2001introduction}. Eq.\ref{eq:1} can be written in matrix form as:
\begin{equation}
[P]=[\Phi][\Omega],
\label{eq:4}
\end{equation}
where $\Phi_{i,j}=\alpha_{i,k}\beta_{j,l}$, while $P$ is an $r\cdot s\times 3$ matrix containing the 3D coordinates of the range map points, $\Phi$ is a $r\cdot s\times n\cdot m$ basis function matrix containing all the products of $\alpha_{i,k}(u)$ and $\beta_{j,l}(w)$, and $\Omega$ is a $n\cdot m \times 3$ matrix of control point coordinates. Thus, the $B$-Spline surface approximation is obtained by solving {Eq.~\ref{eq:4}} as a least-square problem.
%\begin{equation}
%[\Omega]=[[\Phi]^{T}[\Phi]]^{-1}[\Phi]^{T}[P].
%\label{eq:5}
%\end{equation}

Finally, we use control points $\Omega$ as the local surface representation which is a subset representation of the total set of surface points $P$. In our experiments, a 3rd order uniform open knot vector $[0~0~0~0~1~2~2~2~2]$ is used to compute the bases functions. Each patch is represented by $5\times 5$ control points. Since the control points are distribute uniformly in the $x,y$ plane, only 25 depth values are used for the descriptor. In our approach, the BSP descriptors are extracted densely on wrinkles (ridges), instead of extracting them uniformly across the clothing, since our objective is to describe the 3D shape of wrinkles (Section{~\ref{sec:si}}).

%\subsubsection{Local Binary Pattern (LBP)}
%Though LBP has been extracted in the global form, we also extract it in dense local patches in order to enhance the robustness of poorly-stereo-matched regions because of occlusion. In our implementation, LBP are extracted in 32 $\times$32 patches, densely sampled every 16 pixels in both x-y directions. Similar with the global LBP, descriptors are also extracted on another two coarser scales and the size of patches and sampling step are also reduced correspondingly.%

%\subsubsection{Shape Context (SC)}
%Shape Context \cite{} is a local 2D shape stamp which has been applied to deformable shape matching and objects (contours) recognition. More specifically, a shape content is a bi-dimensional histogram of the distances and directions between the centre point and the contour points in a local region. We extract the shape content descriptors on clothes contours (obtained by segmentation), in order to describe the visible components e.g. collars, sleeves, corners etc. Shape content descriptors performs greatly on deformable clothes components due to its tolerance of shape deformation. Need a Fig. ? here.%
%where the weight of each atom can be between 0 and 1. The sum of weights is constrained to be equal to 1 and sparsity is enforced so that most weights are 0.

\subsubsection{Locality-Constrained Linear Coding}
The Bag-of-Features (BoF) technique only projects a descriptor to its nearest atom in the codebook. Sparse coding allows the local descriptor to be represented by more than one codebook atom. Compared to traditional L1-norm sparse coding~\cite{lee2006efficient}, Locality-constrained Linear Coding (LLC)~\cite{wang2010locality} adopts a locality based constraint to enforce sparsity which has been shown to perform more effectively and efficiently in many object recognition tasks. In this paper, we modified the LLC loss function as:
\begin{equation}
\centering
\begin{split}
\min_{C} \sum_{i=1}^{N}\Vert x_{i}-c_{i} B \Vert^{2} + \lambda \Vert x_{i} B^{T} \cdot \omega \odot c_{i} \Vert \\
s.t.~  \sum_{p=1}^{N}c_{i}^{p} = 1, w\textbf{1} = 1, \forall i
\end{split}
\end{equation}
where N is the number of descriptors, $B^{K\times D}$ is the codebook (generated by $K$-means clustering, $D$ is the dimension of the BSP descriptor), $W$ is the weight of the atoms and $c_{i}^{1\times K}$ is the code of the $i$th descriptor, $x_{i}^{1\times D}$. $\odot$ refers to element-wise multiplication. The above loss function treats all codebook bases equally while coding. Our goal is to retrieve the most relevant codebooks learned. Codebook atoms are therefore weighted by a automatic relevance term. The most relevant bases will have a larger $\omega$ value, while less relevant bases will have a smaller $\omega$ value.

where, N is the number of descriptors, $B^{K\times D}$ is the codebook (generated by $K$-means clustering, $D$ is the dimension of BSP descriptor), $c_{i}^{1\times K}$ is the code for the $i$th descriptor, $x_{i}^{1\times D}$.  $\odot$ refers to element-wise multiplication. $d_{i}$ is the Euclidean distance between $x_{i}$ and the codebook atoms, $\omega=\{\omega_{1},...,\omega_{K}\}$ is the weight of the atoms, calculated by: 

\begin{equation}
\centering
\omega_{j} = \frac{1}{1+e^{-\sigma (n_{j}-\bar{n})}}, 
\end{equation}

where $n_{j}$ is the number of descriptors assigned to the $j$th $K$means cluster, and $\bar{n}$ is $N/K$. In our implementation, $\sigma$ is set to $0.5*10^{-2}$ based on practical experience. The motivation of weighting codebook atoms is based on the assumption that the patterns from smaller clusters are more distinctive than those from large clusters. The weights of atoms are set as the sigmoid function of the size of corresponding clusters, in this case, the descriptors will be pushed away from the large clusters and pulled close to the small clusters.

The first term of the loss function is the implicit function of $W$. If $W$ changes while optimising it, the selected codebook bases for coding will also be different. In order to overcome this problem, we first set $W$ with constant values $diag(1,\cdots,1)$, and get the codes $\{c_{i}\}_{i={1,\cdots,N}}$. Then we fix the codes, and optimise $\omega$. Thus, instead of optimising the original parameters, the logarithmic of parameters are optimised in order to convert the constrained $W$ and $\gamma$ to unconstrained values. BGFS\cite{shanno1985broyden} is employed to solve the unconstrained optimisation of $W$. Multiple random starting points are initialised in order to avoid local minimums. $W$ is fixed thereafter in order to retain LLC-coding efficiency.

LLC retrieves a very small number $k$($\ll$ $K$)\footnote{From empirical validation, we found that a $k$ value of 5 works well in practice.} of codebook atoms which are relevant to the matched descriptor. LLC then generates codes in the local coordinate from the retrieved codebook atoms. Sum-pooling is used to generate the global representation:
%That is, once $k$ dictionary atoms are selected, the locality constraint $\lambda (\omega\cdot d_{i}) c_{i}^{T}$ can be neglected, and the code $c_{i}$ can be approximated by solving the linear problem $\min_{c_i}\Vert x_{i}-B c_{i} \Vert^{2}$. Finally, we can get the sparse code $c_{i}$, in which only $k$ dimensions are non-zero and the sum of $\sum_{j=1}^K c_{i}(j) = 1$.
%begin{equation}
%maxpooling:~ c_{out} = max (c_{1},...,c_{n})
%\end{equation}
\begin{equation}
sumpooling:~c_{out} = sum (c_{1},...,c_{n})
\end{equation}
where, $\{c_{1},...,n_{c}\}$ are the input codes, and, $c_{out}$, the final output $LLC$ code. Sum-pooling is calculated for each dimension of the input codes.

\subsection{Classification\label{sec:svm}}
In this paper, we investigate the performance of state-of-the-art classification algorithms as described in Section \ref{sec:class_perf}. We employed SVM with linear and RBF kernels, Random Forest, Gaussian Process for multi-class classification. We found that SVM with RBF kernel provides the best performance among the surveyed classifiers. In our implementation, LibSVM~\cite{libsvm01} is used and a One-Against-All strategy is used for multiple-class classification.

